Enabling Topological Planning with Monocular Vision

Topological strategies for navigation meaningfully reduce the space of possible actions available to a robot, allowing use of heuristic priors or learning to enable computationally efficient, intelligent planning. The challenges in estimating structure with monocular SLAM in low texture or highly cluttered environments have precluded its use for topological planning in the past. We propose a robust sparse map representation that can be built with monocular vision and overcomes these shortcomings. Using a learned sensor, we estimate high-level structure of an environment from streaming images by detecting sparse vertices (e.g., boundaries of walls) and reasoning about the structure between them. We also estimate the known free space in our map, a necessary feature for planning through previously unknown environments. We show that our mapping technique can be used on real data and is sufficient for planning and exploration in simulated multi-agent search and learned subgoal planning applications.

==> old_text.tex <==

\newpage

\section{Introduction}
\label{sec:pd:introduction}

% Potentially missing motivation:
% - Camera + learning as primary sensor / not using a range sensor.
% - We *only* use the sparse detected vertices for the map building and navigation (no other sensor).
% - The visibility graph is good for known environments, but lacks the ability to track unknown space necessary for optimal navigation and exploration in unknown spaces.

TODO: Broad overview of a motivating scenario we solve\wsnote{Will include an overview of a scenario the robot might encounter; see the results section for our ideas.}.

Imagine a robot tasked with navigating a large environment, building a map as it travels. To reach its goal, the agent must plan to enter unknown parts of the map, and in so doing, reason about which areas are unexplored. 
% A cornerstone of the ability to explore is keeping track of regions that are unexplored.
Most planning algorithms deal with this problem by simply assuming all unknown space is free, and so don't need to consider extracting higher level actions from their map, such as rounding one corner versus ansother. Recently however, new approaches to navigation in partially explored environments consider entering unknown space in different areas as explicitly different high-level actions in order to reason about the implications of these actions [cite learned subgoal planning]. Implicit in these approaches is the ability to extract higher level actions from some map representation of the environment in a way that guarantees all possible options are considered. For simple cases where the only actions that are available to the robot are entering unknown space in a 2D occupancy grid, this problem can be solved by manipulating the map after it has been built. However, as the action space becomes more complex, or the sensors available to build a map change, how to decide what constitutes an action becomes less clear. Consider the map output by a modern feature based SLAM system such as ORB-SLAM. While dense visual features are very useful for the task of building a map for localization, reasoning about higher level actions in a map like this is difficult, if not impossible\note{gjstein}{This is a great place to point out that none of these other approaches are robust to outliers, and put too much emphasis on the accuracy of the detector to make maps that are useful (or sufficiently noise-free) for navigation.}.
 
To enable this desired behavior, the agent must construct a map as it navigates that includes (1) a means by which the agent can traverse the known portion of the map and (2) a way of keeping track of regions of space that have not yet been explored. One way to construct such a map could involve dense records of the robot's history of poses and observations (e.g., occupancy grids), however these representations pose significant and expensive data association challenges, and limit the set of actions to simple navigation. In structured environments, like polygonal worlds, detecting geometric landmarks is often suitable for constructing a more sparse map representation --- a graph of polygonal vertices and the walls that connect them --- to enable efficient navigation and exploration.

In known 2\textsc{d} polygonal environments, \emph{reduced visibility graphs} are minimally sufficient representations for navigation\todo{gjstein}{Citation for (reduced?) visibility graph being optimal.}, however this map is usually constructed offline and is not suited for exploration tasks: these representations lack an ability to track \emph{unexplored space}. Gap Navigation Trees~\cite{tovar2007gapnavigation} extend visibility graphs to exploration by constructing a minimal map representation of gap detections and traversed space.  The resulting tree-structured map is designed with navigation-under-uncertainty in mind: the map's \emph{unexplored nodes} correspond to detected gaps the robot has never revealed, and each of these special nodes corresponds to a route through which the robot can enter unknown space in an effort to find the unseen goal. However, Gap Navigation Trees are notably limited to navigation in simply-connected environments~\cite{murphy2008using} and require an infinitely-precise, noiseless sensor, thus limiting its utility in practice.

In this work, we propose a method\note{vpreston}{Maybe not the right wording} for generating a novel, sparse map representation online that encodes the actions available to a robot in an environment from a learned \emph{vertex sensor} to enable efficient navigation in unknown polygonal environments. Instead of storing visibility edges, our \emph{structure-graph} tracks both vertices and the wall-edges that connect them to represent obstacles. This allows us to keep track of \emph{unexplored nodes} like those in the Gap Navigation Tree, which correspond to space that has yet to be explored. 



%In addition to storing traversability edges\note{vpreston}{Is ``traversability edges'' a vocab term that needs to be defined before using it?} in known regions of the map, our \emph{partial reduced visibility graph} \note{cbradley}{We need a unique name for our map representation. Potential options: Obstacle-Graph, Action-Graph, Invisibility-Graph, Wall-Graph, Expanding-Graph, Exploration-Graph, structure-grapyh. I think my favorite is Exploration-Graph}

To generate our representation, we hypothesize the underlying structure of obstacles in the environment by using a Convolutional Neural Network ({\sc{}cnn}) to detect vertices in panoramic images and estimate an additional property we refer to as the vertex orientation --- namely whether or not a vertex is observed as a \emph{gap} in the frame of the robot from panoramic images. From these sparse detections alone we can estimate the presence of walls connecting neighboring vertices, which are ultimately used to infer which regions of the map have yet to be explored. With this data structure, the robot is capable of escaping dead-ends and navigating to other unexplored regions of the map in an effort to reach the unseen goal. Furthermore, the vertex sensor is trained to avoid recognizing smaller objects (clutter) as vertices, enabling a much more compact map than would be possible from structure-based sensors like \textsc{lidar}, without sacrificing navigation performance. 

% By estimating an additional property we refer to as the vertex orientation --- namely whether or not a vertex is observed as a \emph{gap} in the frame of the robot --- we can estimate the presence of walls connecting neighboring vertices, which are then used to infer which regions of the map have yet to be explored. With this data structure, the robot is capable of escaping dead-ends and navigating to other unexplored regions of the map in an effort to reach the unseen goal.

%In this work, we introduce a generalization of the reduced visibility graph that can be constructed online, thereby enabling efficient navigation through unknown environments \note{cbradley}{This feels like it is really under-selling what we are doing. By incorporating walls, we are doing more than constructing the visibility graph (though yes we can extract the visibility graph from the map we build).}. In addition to storing traversability edges\note{vpreston}{Is ``traversability edges'' a vocab term that needs to be defined before using it? Perhaps somewhere in this ``background'' section we ought to take time to explain the features of the graph?} in known regions of the map, our \emph{partial reduced visibility graph} has special \emph{unexplored nodes} as in the Gap Navigation Tree, that correspond to space that has yet to be fully revealed. Equipped with a so-called \emph{vertex sensor} \note{cbradley}{Not sure I love the terminology of ``vertex sensor.''  If we do go this route, I think it's important to emphasize why we care about vertices as they relate to actions (assuming that is still a narrative we care about)}\note{vpreston}{I think that before we launch into ``what we did'' it would be great to add a paragraph which motivates the idea of using camera(s), and extracting information from cameras in order to generate these representations...}, which returns a list of all polygonal vertices in view of the agent,  our agent is capable of constructing a partial reduced visibility graph as it navigates. By estimating an additional property we refer to as the vertex orientation --- namely whether or not a vertex is observed as a \emph{gap} in the frame of the robot --- we can estimate the presence of walls connecting neighboring vertices, which are then used to infer which regions of the map have yet to be explored. With this data structure, the robot is capable of escaping dead-ends and navigating to other unexplored regions of the map in an effort to reach the unseen goal.

% In this work, our agent is equipped with a so-called \emph{vertex sensor}, which returns a list of all polygonal vertices in view of the agent, that we use to construct a \emph{partial reduced visibility graph} as it navigates. When a polygonal environment is fully known, the reduced visibility graph is a minimally sufficient representation for optimal navigation. Yet visibility graphs are traditionally constructed offline\note{gjstein}{I have yet to look into any literature that tries to construct a visibility graph online; I'm certain it will be relevant.} and when navigating in an unexplored environment, such a data structure is not available. In addition to estimating the connectivity between nodes, 

% The graph itself consists of the vertices that make up the polygonal obstacles (the nodes in the graph) and connections between each pair of vertices that share direct line of sight (the graph edges).
The primary contribution of this work is to enable navigation and exploration of unknown environments through the construction of a sparse navigation-aware map from visual input. Our map representation enables optimal\wsnote{This is a suspicion of ours, but is an unsubstantiated claim for now.} navigation of unknown, polygonal environments. We present a posterior over maps that we can sample to obtain the most likely map from a sequence of inherently noisy detections of sparse landmarks estimated from panoramic images\todo{gjstein}{Describe the results; obviously, the results do not yet exist, but describing what results we hope to see is a useful exercise.}. We show that our map representation and estimation procedure is sufficient for navigation/exploration in both simulated and real-world environments. Tentative outline:

\begin{itemize}
    \item Sec.~\ref{sec:pd:navigation-of-unknown} motivates our sparse map representation and details how our agent uses the map to navigate through and explore the unknown environment.
    \item Sec.~\ref{sec:theory} describes how the agent constructs this map online as it navigates; the map-building process involves both evaluating the likelihood of a proposed map (Sec.~\ref{sec:theory:posterior}) and how we sample over possible maps to quickly obtain the most likely map (Sec.~\ref{sec:theory:sampling}).
    \item In Sec.~\ref{sec:theory:learning} we discuss the structure of the {\sc{}cnn}, explain how it is used to estimate vertex detections, and show its predictions in some of our simulated environments.
    \item In Sec.~\ref{sec:results} we demonstrate the performance of our mapping procedure on a variety of navigation and exploration tasks in different environments.
\end{itemize}

\begin{comment}
\subsection{Contributions}
\begin{itemize}
    \item Sparse map representation that can be used to navigate/explore optimally(?)
    \item Posterior over maps given representation allowing us to fuse noisy vertex observations
    \item Learned sensor from vision
    \item Result: TBD
\end{itemize}
\end{comment}

\section{Navigation of Unknown Environments from Sparse Graphs}
\label{sec:pd:navigation-of-unknown}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/fig_orientation_and_planning.jpg}
    \caption{On the left, we show how the \emph{vertex orientation} class is related to the underlying map geometry. The orientation is used during map construction to estimate the existence of wall edges between observed vertices. On the right, we show an example of a map being constructed as an agent travels. Vertices for which only one wall edge exists are considered \emph{unexplored}, since all vertices must be connected to two edges in a polygonal environment.}
    %\label{fig:orientation-and-planning}
\end{figure}


% The goal of this section is to (1) describe what our sparse map representation looks like (after sampling) and (2) how we can use this sparse map for navigation. The key idea here is to motivate how we use the walls to determine which vertices are 'subgoals' (correspond to unexplored space). At the top of the second page, I'll need a figure that shows 2 things: (Left) how we can use the vertex orientation to estimate where walls exist and (Right) some sample maps that show how we estimate which nodes are unexplored (a step-by-step diagram would be useful here).

As established in the previous section, navigation through an unknown environment requires a map that (1) enables traversal of known space and (2) a means of keeping track of regions of space that have not yet been explored. In this section, we motivate our sparse map representation and describe how it can be used to efficiently navigate through unknown environments.

Our map is a graph in which nodes correspond to detected landmarks --- each a vertex in the underlying polygonal representation --- and edges are walls. As the agent navigates through the environment, it reveals new vertices and adds them to the map. Similarly, we can infer the presence of walls once both of its vertices have been observed in tandem\todo{gjstein}{We probably want a footnote here mentioning that the walls are, in fact, oriented: i.e. we know what side of a wall we are on. We can mention that, while not necessary when sensing is perfect, using oriented walls is important for fusing noisy sensor measurements.}. 

As the map is revealed and vertices are added to the graph, vertices with only a single observed wall should\note{vpreston}{could?} be considered \emph{unexplored}, since all vertices must be connected to two walls in a polygonal environment. Each unexplored vertex corresponds to a \emph{high-level action}: the robot navigates to a vertex and explores the space beyond it in either an effort to reach the goal, in goal directed navigation, or reveal the environment, for exploration tasks. This continues until the goal is reached or the map is fully revealed. We see this behavior in the right plot of Fig.~\ref{fig:orientation-and-planning}, in which the robot seeks to explore the environment by navigating towards unexplored nodes. For more complex environments, a visibility graph can be computed from the map so as to enable efficient traversal of known space.\feedback{gjstein}{What else needs to be added to this section? I think some of the language we talked about along the lines of \emph{visibility graphs alone are insufficient because we need to keep track of unknown space} belongs here.}\feedback{vpreston}{I agree with adding the language you suggest.}

Once the agent has selected a high-level action, it plans a trajectory towards the corresponding node. To do this, we generate a visibility graph in the known portion of our map, which easily done using ray-tracing for collision detection between nodes, and generates a trajectory towards the node of interest. To follow this trajectory, the agent uses a pure pursuit controller and an onboard depth sensor\wsnote{The exact nature of this depth sensor is yet to be determined. We could use something like MonoDepth to estimate local obstacles directly from the panoramic images or would be provided by another onboard sensor. So long as we can reactively navigate towards a distant (perhaps unseen) waypoint and avoid local, convex obstacles, we can plan.} to navigate towards each waypoint along the path. With this approach, our system is capable of not only navigating towards vertices, but also avoiding local convex obstacles, like clutter, that we do not want\note{vpreston}{Maybe delete?} to include in the graph.



% It is straightforward to generate a visibility graph from the map.
% Greedily navigate towards the goal, revealing new vertices and walls as we travel.
% One notable failing of visibility graph is that visibility edges are not the same as the path a physical agent must take; (We will likely need to make some claims about the performance of the agent. This may involve some sort of "inflation radius" in the visibility graph, or at least the assumption that the distance between vertices is never sufficiently small as to prevent the robot from traveling through the space.)
% 

% Why do we need to keep track of unknown space? Metric-goal-directed navigation doesn't need it, so we need to do more things.


\section{Theory: Estimating the Most Likely Sparse Map}
\label{sec:theory}

Having established how we can use our sparse map representation for navigation, we can now discuss how such a map can be constructed online using sparse sensor observations. This section is devoted to a discussion of our map-building process, in which we sample the posterior distribution of maps --- conditioned on the sparse, noisy observations of polygonal vertices --- in order to recover the most-likely polygonal map representation. The agent is equipped with a \emph{vertex sensor}, which returns a list of all vertices visible, in any direction, from the agent's current position. The domain of each \emph{vertex detection} is $ \text{[position + covariance]} \times l$ where \footnote{TODO(gjstein):Define the domain of a \emph{position + covariance}} and \(l \in \text{[4D simplex]}\) is the estimated vertex orientation, itself a point on a 4\textsc{d} simplex. Each observation $z$ is a list of vertex detections $\sigma$, ordered by the angle at which it was observed; the relative angle of detections within a single observation will be used in later sections. The sensor itself is fundamentally noisy, so each observation may have extraneous landmark detections --- false positive detections --- or missing detections --- false negative detections --- each with a known rate of occurrence.

We can use the noisy sensor observations to construct the map. As we navigate, we grow the set of detected polygonal vertices and walls that connect them, which we can then use to propose possible maps of the underlying environment. The goodness of a proposed map is given by its posterior likelihood: Sec.~\ref{sec:theory:posterior} is devoted to a discussion of this likelihood. Sec.~\ref{sec:theory:sampling} includes a discussion of how individual vertex detections are associated with one another. It also includes a discussion of how sensor observations are combined into to form the set of possible maps, from which proposed maps can be sampled (discussed in Sec.~\ref{sec:theory:sampling-possible-maps}).

% Having established how we can use our structure graph for navigation, how do we fuse sensor observations to build such a map online? This section is devoted to a discussion of our map-building process, in which we estimate the most-likely polygonal world map from noisy observations of polygonal vertices. 

% Using these sensor observations, we estimate the likelihood of a proposed map in the hopes of discovering the most likely underlying map given our observations. A map is defined by a set of vertices and a set of walls that connect the map's vertices. We represent a map \(m\) \todo{gjstein}{How do we write out the domain over maps? Each set (vertices and walls) are arbitrarily long, so how do we notate that?}. \footnote{TODO-RESPONSE(vpreston): Perhaps looking at how this is done with Dirichlet Processes or Gaussian Processes is the right move? These are theoretically infinite-dimensional systems....}. \footnote{TODO(gjstein): walls are 'ordered sets'. I know why this is important, but I don't know how to motivate this just yet.} In Sec. [??], we define the posterior likelihood over maps given a series of sensor observations. Yet iterating over all possible maps is computationally infeasible, and so in Sec. [??] we discuss how we can efficiently construct a proposal distribution that we use in combination with particle filtering to more quickly determine the most likely state of the world.

% \emph{Vertex detections} are two-element tuples, consisting of the relative position and an additional property we refer to as the \emph{vertex orientation} \note{cbradley}{orientation, label, class, type. These are apparently our options for referring to this property. I don't have a preference (concerns about ``yaw'' for orientation)}: depending on the angle at which the robot views the walls connected to a particular vertex, a detection falls into one of four possible orientation classes.

\subsection{Form of the Posterior over Maps}
\label{sec:theory:posterior}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/fig_simple_hallway_map_progression.png}
    \caption{This figure shows how we construct a map online. The second row is a visualization of the domain of possible maps: yellow circles correspond to potential vertices, while edges represent walls and are colored from red-to-green to represent the estimated likelihood the wall exists. We use {\sc{}mcmc} sampling to fuse vertices --- as in \texttt{(b)->(c)} --- which is helpful when initial data association fails (see Sec.~\ref{sec:theory:sampling}). We sample over the map domain, enabling and disabling potential walls and vertices, to determine the most likely map as the robot travels (see Sec.~\ref{sec:theory:posterior}). By the end of travel \texttt{(e)}, the estimated map closely matches the underlying geometry; erroneous vertex detections do not appear.}
    \label{fig:simple-sim-hallway-results}
\end{figure}


% Formal definition of a map (this might be done in section 2; unsure)


% Form of the posterior: split into terms we understand.
The posterior over maps can be expanded as follows using Bayes Rule:\todo{vpreston}{May want to consider adding a table for notation}
\begin{equation}
\log P(m | z^1, \cdots, z^N ) = \sum_{i=0}^N \log P(z^i | m) + \log P(m) - \log P( z^1, \cdots, z^N )
\end{equation}

where $z$ represents an observation, $m$ represents a map, and we have assumed that the sensor observations are i.i.d to factor $\log P(z^1, \cdots, z^N | m)$. The final term, the likelihood of a sensor measurement, is a constant and can be ignored. The prior distribution over maps, $P(m)$, is intractably difficult to obtain in practice. Yet we can use this term to incorporate some global priors about the map, namely biases against the addition of new vertices and walls, which helps to eliminate false positive landmarks.\todo{gjstein}{Add an equation for the expanded form of $P(m)$. ``This requires that multiple positive observations are needed for each before they are added to the map, thereby reducing the number of false positive landmarks.''}

% ; however we can use this term to incorporate some global priors about the map in order to compensate for the existence of false-positive values. We include a prior that biases against the creation of new nodes and walls; this should eliminate false-positive vertices or walls which have few positive detections. (I'm going to need a better way to explain/sell this idea; I have no doubt people will understand why we want this, but I should look in the literature [SLAM perhaps?] to see how this is motivated or argued for.)

The likelihood of a sensor observation $P(z^i | m)$ is at the heart of the posterior distribution. To compute this likelihood, we generate a \emph{hypothetical observation} $z^i_h$ from the robot's position at time $i$, $x^i$, and compare it to the real observation $z^i$. Hypothetical observations are generated by ray-casting the underlying vertices to the sensor onboard the robot; vertices for which the ray is not obstructed by walls are added to the list of detections. As for the real vertex detections, each hypothetical detection $\sigma_h^{i,j}$ has its own \emph{vertex orientation} --- computed, as in Fig.~\ref{fig:orientation-and-planning}, from the geometry of the proposed map and the robot position $x^i$. Since the hypothetical observation is a sufficient statistic of the map $m$ at position $x^i$, the likelihood can be rewritten $P(z^i | m) = P(z^i | z_h^i)$. 

Each observation, both actual and hypothesized, consist of a set of vertex detections: $z^i = \{\sigma^{i,0}, \cdots, \sigma^{i, N_i} \}$. Upon compaing the two, detections fall into three types:
\begin{description}
    \item[Associated Detections] A list of two-element tuples, each a pair of observed/hypothetical vertex detections that correspond to one another. After data association, the likelihood of a match between an observed and a hypothetical vertex detection is a function of their respective \emph{vertex orientation} (class)\todo{gjstein}{Mention that point vertices exist, which return a ``fake value'' on the simplex or a [0,0,0,0] value; unsure which for the moment.}. The likelihood of a detected pair is computed using the dot product, $l \cdot l_h$, where $l$ and $l_h$ are the vertex orientations for the detected and hypothetical detections respectively. Unfortunately, a sufficiently incorrect vertex prediction can result in an asymptotically low probability; as such, we include a lower bound $p_l$ on the likelihood of any associated detections. Combined, this becomes $P(\theta, \theta_h) = \max(l \cdot l_h,\, p_l)$.
    \item[False Positives] A list of length $N_p^i$ of observed detections that do not have a corresponding hypothetical vertex. False positives occur according to the false positive rate: $R_\text{fp}$.
    \item[False Negatives] A list of length $N_n^i$ of hypothetical detections that do not have a corresponding observed vertex detection. False negatives occur with a rate $R_\text{fn}$.
\end{description}

With these types, we can write out the full posterior likelihood of a proposed map:
\begin{equation}\label{eq:posterior-final}
    \log P(m | z^1, \cdots, z^N) = \sum_{i=0}^N \text{TODO: Need notation for data association.}
\end{equation}


% To evaluate $(P(\theta_i | \theta_{h}(x_i, m))$, we associate the vertices (already done using the MH-distance). Note: I have no idea what the notation for this looks like, but the data association should return three sets: (1) false positives: a list, of length \(N_p\), of observed vertex detections that do not correspond to any hypothetical vertex detections; (2) false negatives: a list, of length \(N_f\) of hypothetical vertex detections that do not have a corresponding observed detection; (3) associated vertices: a list, of length \(N_a\) of 2-element tuples, each an observed-hypothetical pair that correspond to one another. (It is likely convenient to say that this actually returns two lists \(G_o\) and \(G_h\) that contain indices of the matching pairs from the corresponding observations.) Now: $$ P(\theta_) = \prod_{i=0}^{N_a} P(\theta_{o, G_o(i)}, \theta_{h, G_h(i)})  \cdot N_ $$


% Talk about data association + false positive/negative detections
% Discuss how the vertex orientation is computed and how it is used to determine the likelihood of a paired set of detections.
% Describe how the vertex orientation is used to determine the orientation of a vertex.

This posterior codifies a number of behaviors we would expect to see during our map-building process. First, the posterior allows us to rule out false positive vertices in a principled manner. Since false positive vertices can result in unwanted false negative observations as the robot travels, it ultimately makes it more likely that the vertex does not appear in the underlying geometry. Second, the existence of a wall depends on both its ability to occlude vertices \emph{and} the impact it has on the orientation (class) of the hypothetical vertices to which it connects. By occluding portions of the map, the walls also determine\note{vpreston}{this is a weird word choice to me} the number of false positive and false negative detections.


% \begin{itemize}
% \item\relax [I need to point out that the number of false positives and negatives will depend on the presence of walls; the hypothesized measurements respect walls/obstacles. Important to reinforce this idea, since it's one of the more expensive operations; it's possible we may have to turn this off, though, since it might be prohibitive even with sampling.]
% \item Each observation, both actual and hypothesized, consist of a set of vertex detections \note{vpreston}{Which is at least range and bearing. So far we haven't explicitly considered how to include vertex class as part of the inference regime (since this is a local measurement)}. To evaluate \(P(\theta_i | \theta_{h}(x_i, m))\), we associate the vertices (already done using the MH-distance). Note: I have no idea what the notation for this looks like, but the data association should return three sets: (1) false positives: a list, of length \(N_p\), of observed vertex detections that do not correspond to any hypothetical vertex detections; (2) false negatives: a list, of length \(N_f\) of hypothetical vertex detections that do not have a corresponding observed detection; (3) associated vertices: a list, of length \(N_a\) of 2-element tuples, each an observed-hypothetical pair that correspond to one another. (It is likely convenient to say that this actually returns two lists \(G_o\) and \(G_h\) that contain indices of the matching pairs from the corresponding observations.) Now: $$ P(\theta_) = \prod_{i=0}^{N_a} P(\theta_{o, G_o(i)}, \theta_{h, G_h(i)})  \cdot N_ $$
% \item The likelihood of two detections matching one another is simply how similar the estimated vertex orientation \note{vpreston}{I'm confused here -- doesn't orientation refer to class of vertex? In this case, is it more clear to discuss ``metric orientation''?} is to the hypothesized vertex orientation, which can be easily computed using the dot product: \(P(\theta_o, \theta_h) = l_o \cdot l_h\).
% \item We also want a "floor" value associated with each of these. If the match is sufficiently poor, we recognize that the more likely scenario is that the data association was unlikely, and we replace the match with \(R_p \cdot R_n\), the likelihood of a combined false positive / false negative.
% \end{itemize}

\subsection{Data Association\note{vpreston}{Maybe ``Vertex Association''?}}
\label{sec:theory:sampling}
The posterior over maps gives us the ability to determine which of two maps is more likely given a set of sensor observations. To evaluate Eq.~\eqref{eq:posterior-final} we require the ability to cluster vertex detections across observations to form map proposals: clusters of vertex detections yield \emph{potential vertices} from which we can sample to get potential maps.

As new observations are added online, we use Mahalnobis distance as presented in \cite{murphy2008using} to associate detections. As new vertex detections are generated, their estimated metric locations are compared with metric locations of vertices in the graph. A new detection is associated with an existing vertex if the vertex is within two standard deviations of the detection's estimated covariance. Successful associations are ultimately used to update the vertex position and covariance by using an Extended Kalman Filter \todo{vpreston}{Add reference}. Detections which are unassociated with an existing vertex create new vertices in the graph, under the constraint that no two detections from a single observation can be associated with a single cluster.

%Proposing a map graph from vertices is as simple as deciding, based on the vertex type at time of detection, which vertices should have walls between them for a given detection, then considering the probability of that wall for each detection that could have see it if it were there.

% This initial step significantly reduces the dimensionality of a proposed graph, however will fail to handle all sensor noise or false detections.\note{vpreston}{maybe a figure motivating this case?} We use a Markov-Chain Monte-Carlo (\textsc{mcmc}) sampling procedure, modified from \cite{ranganathan2006bayesian} to propose clustering vertices together. Our modification of the presentation in \cite{ranganathan2006bayesian} lies primarily in the definition of the likelihood of the data given metric vertex locations and proposed vertex clusters:\wsnote{We suspect that the method we describe here may change significantly moving forward.}

% \begin{equation}\label{eq:obslike-mcmc}
%     - \log P(Z|X,T) = \left(\frac{||X-X_z||}{\sigma_z}\right)^2 + \sum_{S \in T}\sum_{i, j \in S}\left(\frac{||(X_{i} - X_{j}||)}{\sigma_t}\right)^2 + \sum_{S \in T}\sum_{i, j \in S}\left(\frac{d(X_{zi}, X_{zj})}{\sigma_t}\right)^2 
% \end{equation}

% where $Z$ is the set of vertices from the association performed by the Mahalanobis distance, $X$ is the set of metric vertex locations and is found through an optimization regime described in \cite{ranganathan2006bayesian}, $T$ is the proposed clustering of vertices, $X_z$ is the set of observed vertex locations, and $S$ is a cluster of vertices. Parameters $\sigma_z$ and $\sigma_t$ capture the amount of error tolerable for the difference in cluster metric locations and observed metric locations, and error in cluster associations, respectively. The function $d(\cdot,\cdot)$ is the Bhattacharyya distance between the inputs. The first term of the likelihood captures the idea that the metric locations of a proposed topology should not lie far from the observations. The second term captures the idea that within a cluster, vertices should lie close together, and the third term specifically considers whether the distributions between clustered observations feasibly overlap.

%and motivated by the methods in [GREEN's RJMCMC PAPER]\todo{vpreston}{Add Green's RJMCMC paper to cite for this method (contains the proof for detailed balance in partition spaces} over the distribution of vertices to propose merging vertices together. 

%We treat the space of possible vertex combinations as a set of partitions. The proposal distribution from which to draw a partition set considers one of two moves: merging two partitions together, and splitting partitions of more than one vertex apart. The proposal acceptance ratio is merely a function of the number of different merge and split combinations. The posterior distribution, or the probability of a proposed set of vertex partitions given the vertex locations and covariances, can be expanded using Bayes Law:

% \begin{equation}\label{eq:posterior-mcmc}
%     P(T|O) \propto P(O|T)P(T)
% \end{equation}

% where $T$ represents the proposal vertex partitions and $O$ represents the vertex observations (position and covariance). For simplicity, we assume an uninformative uniform prior over the space of proposal vertex partitions. The likelihood of the vertex observations given a proposal vertex partition can be evaluated as:

% \begin{equation}\label{eq:likelihood-mcmc}
%     P(O|T) = \int_X P(O|X,T)P(X|T)
% \end{equation}

% where $X$ represents the topology-based vertex locations. The prior over vertex locations given a partition set we can use to encode that distinct vertices will tend not to fall close together. We follow the definition of the penalty function, Eqn. 11 and Eqn. 12 from \cite{ranganathan2006bayesian} exactly. The observation likelihood we encode as:

% \begin{equation}\label{eq:obslike-mcmc}
%     - \log P(O|X,T) = \left(\frac{||X-X_O||}{\sigma_o}\right)^2 + \sum_{S \in T}\sum_{i, j \in S}\left(\frac{d(X_{Oi} - X_{Oj})}{\sigma_t}\right)^2 
% \end{equation}

% where $X_o$ represents the true observed vertex locations, $\sigma_o$ and $\sigma_t$ are variances we will tolerate in both location and partition set assignments, respectively, and $S$ represents a set in the partition space $T$. The first term encourages that measured and estimated vertex locations lie close together. The second term encourages that grouped vertices lie close together as well. We define a distance measure, $d(\cdot)$, as the Bhattacharyya distance, which considers both metric location and covariance of the vertices. Our expression for the negative log-likelihood is distinct from that presented in \cite{ranganathan2006bayesian}.

% Generally, we do not know $X$, and will need to estimate it. We perform a simple minimization routine over the first term in Eqn. \ref{eq:obslike-mcmc} to get $X*$, and place a Gaussian distribution over $X*$ in order to perform a Monte Carlo approximation for Eqn. \ref{eq:likelihood-mcmc} according to Eqn. 14 in \cite{ranganathan2006bayesian}.\todo{vpreston}{May need to revisit this section based on an update to this likelihood term we're considering.}

% Running the \textsc{mcmc} sampler yields at most a handful of potential vertex clusters\todo{vpreston}{Maybe some figures/more discussion here about the quality of the sampler?} that we can then check against the map posterior, Eq.~\eqref{eq:posterior-final} to evaluate the likelihood of each proposed map. Because the process of data-association using Mahalanobis distance is reasonably good for a few measurements, we can run the vertex sampler less frequently than the network gives detections. We can optimize the clusters in an ``outer-loop'' that happens at a slower rate, thus enabling the sampler to be used in a real time system. Additionally, by doing this sampling repeatedly over the robot's trajectory, the proposed clusters generally don't stray too far from the correct one. Other savings in computation are made by only considering vertices that were visible by the robot recently, so the whole map isn't sampled over at every step.  Note that to deal with the problem of loop closure, even less frequently than the usual sampler, we occasionally do sample over the entire map. Because this can be done at fairly sparse intervals however, it does not come at a major computational cost.

\subsection{Sampling the Set of Possible Maps}
\label{sec:theory:sampling-possible-maps}

The output of data association is a set of \emph{potential vertices}, of which only a subset may appear in the final map. This set defines the space of possible maps where a proposed map is an inclusive subset of the set of possible vertices and a set of wall edges that connect pairs vertices from the selected subset. We sample over this space and use the map posterior, Eq.~\eqref{eq:posterior-final}, to select the most likely map. Each sampling step\todo{gjstein}{This procedure is not quite done, for now we are only sampling over vertices, not edges, and we only sample one vertex at a time.} we randomly select a potential vertex and either add or remove it from the set of selected vertices. We can then sample walls from the set of edges that connect pairs of selected vertices and similarly enable or disable them.

In general, sampling over both vertices and edges can become rather expensive. To guide the sampling process, we can estimate the marginal likelihood a wall edge exists and use this to bias the sampling process. For a single sensor observation, $z$, the likelihood of a wall edge between two vertices, the left and right vertex observations $\sigma_l$ and $\sigma_r$, depends on their respective orientations, $l_l$ and $l_r$, is given by:
\begin{equation}
P(w_{lr}|z) = P_{\text{fp}}^{N_{\text{fp}}}\left[1 - (1 - P(l_l = \text{right gap}) P(l_r = \text{left gap}) \right]
\end{equation}
where $N_{fp}$ is the number of detections that occur between $\sigma_l$ and $\sigma_r$: if a wall were to exist connecting $\sigma_l$ and $\sigma_r$, any vertex observations between the two endpoints would have to be false positives, and so the likelihood of the wall existing should decrease for every observation we see between the two\footnote{As a result of this false-positive approach, walls must be \emph{ordered}, so that $P(w_{lr}) \neq P(w_{rl})$. This way, if we view a wall from the other side, these false-positive detections do not count against it's existence.}. If two vertices never appear in a single observation, we do not consider adding the wall edge connecting those vertices to the map.






% [ ] Pull discussion of 'remaining vertices' out of the previous section and move it to the beginning here
% [ ] Intro: The vertices from the previous section, after data association and vertex merging, represent all \emph{possible} vertices that may appear in the final map and includes both true vertices and false positives (resulting from our noisy sensor). Only a subset of these vertices may appear in the final map. [Need to transition to this better, to include walls.] This set of possible vertices defines the space of possible maps: a proposed map is an inclusive subset of possible vertices and a set of wall edges connecting any pairs of these vertices. We sample over this space using the posterior defined in [ref section] to determine the most likely map.
% To guide this sampling process, we can compute an approximate likelihood a wall edge exists as the robot travels and use this likelihood to inform the wall sampling process.
% We sample over the set of possible vertices and the set of possible wall edges that connect the selected set of vertices.
% [ ] Walls: In addition to vertices, the final map representation must also include walls. In general, a wall edge may exist between any two vertices, however, we can use our sensor measurements to constrain the set of wall proposals. 
% [ ] We 

% The vertices from the previous section are all the possible vertices.

% This section should probably include a "description" list of the different sampling operations that are possible. These include (1) Vertex toggling (2) Wall toggling and (3) Vertex merging [and splitting?]. 


\section{Detecting Vertices in Images using Convolutional Neural Networks}
\label{sec:theory:learning}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/fig_simple_nn_results.jpg}
    \caption{Here we see the output of the neural network in a simulated hallway environment. In addition to estimating the bearing at which a vertex occurs, the network also estimates the range (plus the range covariance) and orientation (classification) of each vertex, which are then used to construct the map.}
    \label{fig:neural-net-results}
\end{figure}

% Overview: we learn to predict the presence of vertices from panoramic images collected onboard the robot. We train a convolutional neural network to estimate the presence of vertices along with the 
% Network structure: describe/show the structure of the network and the loss function (Which will include a discussion of what the different outputs look like, and how we get a continuous output using a signal that only exists at certain points.
% We use peak detection to obtain the location of the different vertices.

The goal of this work is to enable navigation of unknown environments using vision data. We learn to predict the presence of vertices from panoramic images collected onboard the robot. To do this, we train a convolutional neural network ({\sc{}cnn}) to estimate the likelihood of a vertex existing in a particular direction along with a few other properties: the range of each vertex, the covariance of the vertex range, and the 4\textsc{d} estimated vertex orientation (classification). Our convolutional neural network (\textsc{cnn}) network takes a $128\times 512$ pixel RGB panoramic image as input and outputs the likelihood a vertex exists in the direction of each column (a 512\textsc{d} vector) of the image and a few other properties:  the estimated vertex range (512\textsc{d}), the covariance of the vertex range (512\textsc{d}), and the estimated vertex orientation/classification ($512\times4$\textsc{d}). The network begins with 6 convolutional layers --- of kernel dimension ([3,3,3,8], [3,3,8,16], [3,3,16,32], [3,3,32,64], [5,5,64,128], [5,5,128,256]) --- each followed by a $2\times2$ max-pool layer and batch normalization. Following the convolutional layers, we add 3 fully connected layers each with 1024 hidden nodes and followed by batch norm layers. The output of this encoder portion is fed to four different output layers (each fully connected) with different activation functions: a sigmoid output for the vertex likelihood, a 4-way softmax output for each of the 512 columns of the vertex orientation, and an identity output for each of the range mean and covariance.\wsnote{More network details forthcoming. Still somewhat a work in progress.}


We show the output of our trained network in Fig.~\ref{fig:neural-net-results}. The output of the network includes the \emph{vertex likelihood}, on which we use peak detection to convert the measurement to discrete vertex observations\todo{gjstein}{Should we be using a Gaussian Mixture Model to estimate the location of the vertices? This might also give us a slightly more principled way of getting the peaks out along with an angular covariance. In addition, the area under the curve for each Gaussian might give us a more appropriate confidence metric than what we currently use, which is just the height of each peak.}\note{vpreston}{I think that this could be interesting to consider. I definitely agree that having a more principled way of characterizing the peaks would be useful.}. The network frequently estimates the correct number of vertices in each frame\wsnote{This will be supported by a number (some metric of quality) in a later draft.}, though the network does occasionally suffer from false positive and false negative detections. One notable failure mode occurs when two vertices are nearly colinear, since peak detection is incapable of resolving this situation. We only return only a single vertex, yet the network has learned to associate a large range covariance in this region. Our mapping procedure (Sec.~\ref{sec:theory}) is designed with a noisy sensor in mind, and is robust to occasional errors like these.

\section{Results: Mapping and Navigation in Simulated Environments}
\label{sec:results}

In this section, we demonstrate the capabilities of our  system on a variety of simulated environments.

First, we navigate through a simple simulated hallway environment\todo{gjstein}{I will have mentioned this environment in the neural network section, so I should reference it.}. Fig.~\ref{fig:simple-sim-hallway-results} shows how the map evolves as the robot navigates through the hallway. Our procedure fuses sparse vertex detections and uses our data association procedure to group detections into possible landmarks. Erroneous detections occasionally result in the creation of extra vertices as we travel. During navigation, we run our sampling procedure to determine the most likely map, showing that our sampling-based map-building process is capable of (1) fusing sensor measurements into a sensible \emph{proposal map domain} and (2) sampling over the domain of possible maps to correctly estimate the underlying geometry.

{\bf{}Future Simulated Experiments} The example shown in Fig.~\ref{fig:simple-sim-hallway-results} is a proof-of-concept that our approach is capable of estimating the most likely map. Moving forward to CoRL, we have a number of other experiments we would like to show here is a list of simulated experiments we aim to try:

\begin{description}
    \item[Map-in-the-loop navigation and exploration] For the experiment we've shown so far, the robot's trajectory was predetermined. Next, we will use the online-constructed map to navigate and explore in the simulated hallway environment. For a goal-directed navigation task, we will generate a visibility graph and greedily navigate towards the goal node. We would also like to show that we are capable of undirected exploration: the agent will fully explore the environment until no \emph{unexplored nodes} remain, thus creating a complete map of the environment.
    \item[Cluttered simulated hallway] One of the advantages of using a learned sensor, as opposed to a {\sc{}lidar}-based approach, is that we can avoid adding smaller obstacles (clutter) to our map; this further sparsifies the map and simplifies the map-building process. We aim to add clutter to the hallway environment and show that we can build a map that lacks such elements and navigate between nodes using a reactive policy.
    \item[More complex simulated environments] There are a number of environments we have considered. 
    \begin{enumerate}
        \item A \emph{loopy} hallway environment, one in which the hallway is allowed to double-back and intersect itself, showing that we are capable of building slightly more complex environments.
        \item An office-like environment, with hallways and office structures connected to these hallways.
        \item An outdoor environment, like the Guardian Center map. It would be nice to show that we are capable of constructing a map from relatively spread-out, non-convex obstacles. In addition, the guardian center environment is particularly interesting because we would like to treat smaller obstacles like cars and trees as clutter, showing that we can build a map that only contains the buildings.
    \end{enumerate}
    \item[Learned Subgoal Planning] This is one that we will likely not get to by the submission deadline, but we are pretty excited to use our map representation for Learned Subgoal Planning (our last CoRL paper). Our map has all the elements that framework required and I suspect it would not be particularly difficult to estimate the properties of each vertex/subgoal --- like the probability a path including that vertex would ultimately lead to the goal --- alongside the vertex range and orientation already output by our neural network. It is more likely that we will only include this as a subject of future work in the conclusion of this paper.
\end{description}

{\bf{}Future Real-world Experiments} We also aim to perform experiments in real-world environments. We are looking for suggestions on some real-world places that would be best for this, but here are a few we have in mind:

\begin{description}
   \item[Build a map of part of MIT campus] We aim to revive the GeneSIS-RT work to generate realistic training data for vertex estimation. Hopefully, this will allow us to build a map of a small portion of MIT campus using real data. This is a minimum bar for real-world experiments with this work: to show that we can construct a map offline with real data, and that plans the robot would make with this (possibly incomplete) map are sensible.
   \item[Navigate across MIT campus] This is probably the most ambitious experiment that we have in mind: we would like to build a map of MIT online and navigate across campus, showing that we can solve a real world problem with our planner in-the-loop.
\end{description}

\section{Assumptions and Parameters}


%===============================================================================

% The maximum paper length is 8 pages excluding references and acknowledgements, and 10 pages including references and acknowledgements



\clearpage
% The acknowledgments are automatically included only in the final version of the paper.
\acknowledgments{[todo] This work was supported by the Office of Naval Research and Marc Steinberg under the PERISCOPE MURI Contract \#N00014-17-1-2699. Their support is gratefully acknowledged.}%

%===============================================================================

% no \bibliographystyle is required, since the corl style is automatically used.
\bibliography{sparse_vis_nav}  % .bib

%\clearpage

==> related_work.tex <==

\section{Related Work}
% In the presentation of this paper, we have referenced all key literature directly related to our approach. In this section, we primarily address other works which consider XXX.

[\textbf{Note for Nick: nearly all of this information appears elsewhere at this point. Can we eliminate this section entirely (after we move around a couple of the citations not yet mentioned earlier)?}]
Topology-aware planning has long been a research interest in robotics. [todo: a couple classic refs; probably Ben Keuipers] Topology has been used for navigation in known maps to specify the planning objective (e.g., \emph{reach the goal by going left around the obstacle}~\cite{park2015homotopy}). Specifying planning problems in the language of topology has particular advantages when planning under uncertainty, since grouping trajectories according to some topological property can be used to massively simplify the space of possible actions. Doing so can be used to encode heuristic priors for otherwise challenging planning problems (e.g., that robots should split-up in multi-agent \emph{search and rescue} applications~\cite{govindarajan2016human}) or plan more effectively when there is uncertainty in the presence of obstacles~\cite{bhattacharya2015persistent}.

Of particular interest in this paper is planning through unknown environments, for which relative homology~\cite{pokorny2016topological} can be helpful in enumerating the various ways the robot may leave known space. Gap Navigation Trees~\cite{tovar2007gapnavigation,tovar2004gapnavigation} advanced research in this space, building a sparse --- and, in fact, minimal --- tree-structured map of the world by detecting \emph{gaps}, discontinuities in depth, and maintaining a list of unexplored branches for later exploration. Yet Gap Navigation Trees and derivatives are notably limited to navigation in simply-connected environments or put unrealistic constraints on the noise in the sensor~\cite{murphy2008gntlaser}, thus limiting their utility in practice.

Frontiers, boundaries between known and unknown space, have been used to reduce the action space for planning in unknown environments~\cite{yamauchi1997frontier,Korb2018,tian2018rescue}. Frontier-based approaches involve building an occupancy-grid map of the world using idealized sensors or laser range finders and keeping track of space that has yet to be observed. While not explicitly reasoning about topology, frontiers capture a less-finely discretized notion of \emph{relative homology}~\cite{pokorny2016topological} and similarly define the different ways an agent can enter unknown space. Though some recent work has shown that considering frontiers, as opposed to homology, limits planning effectiveness in some environments~\cite{kim2013topological}, frontiers are often sufficient for effective planning. One recent paper~\cite{stein2018learning} estimates properties of frontiers, including the likelihood the goal can be reached through the boundary of interest, to approximate the expected cost of topological actions, thereby enabling tractable computation of expected cost and demonstrating improvements in planning through unknown environments.

%Topological mapping?
%Coverage based planners?
% To avoid keeping dense records of robot history and observations, sparse maps can be used to efficiently store a sufficient representation of a graph for planning. Reduced visibility graphs have been shown to be minimally sufficient for navigation in known 2\textsc{d} polygonal environments~\cite{tovar2003optimal}, however this map is usually constructed offline and is not suited for exploration tasks because these representations lack an ability to track unexplored space. Gap Navigation Trees~\cite{tovar2007gapnavigation} extend visibility graphs to exploration by constructing a minimal map representation of gap detections and traversed space. The resulting tree-structured map is designed with navigation-under-uncertainty in mind: the map's unexplored nodes correspond to detected gaps the robot has never revealed, and each of these special nodes corresponds to a route through which the robot can enter unknown space in an effort to find the unseen goal. However, Gap Navigation Trees are notably limited to navigation in simply-connected environments~\cite{murphy2008using} and require an infinitely-precise, noiseless sensor, thus limiting its utility in practice.

%Maps produced by state of the art feature-based SLAM methods~\cite{mur2017orb}, use sparse visual features to build dense feature graphs, and are generally optimized for localization tasks. Such maps can be collapsed into occupancy grids in order to use topology aware planning, however the computational challenges associated with principled rejection of outliers makes these maps susceptible to sensor noise [cite RANSAC/Carlone], thus limiting their effectiveness in practice for topological planning strategies. Relatedly, keeping track of unknown space is a critical capability for planning applications in unknown environments, yet is challenging for sparse feature-based SLAM, owing to difficulties in estimating the precise location of occluding obstacles [cite needed]. It is filling these technical gaps that this paper addresses.
